Framing Effects on Privacy Concerns about a Home Telepresence Robot

Privacy-sensitive robotics is an emerging area of HRI research. Judgments about privacy would seem to be context-dependent, but none of the promising work on contextual "frames" has focused on privacy concerns. This work studies the impact of contextual "frames" on local users' privacy judgments in a home telepresence setting. Our methodology consists of using an online questionnaire to collect responses to animated videos of a telepresence robot after framing people with an introductory paragraph. The results of four studies indicate a large effect of manipulating the robot operator's identity between a stranger and a close confidante. It also appears that this framing effect persists throughout several videos. These findings serve to caution HRI researchers that a change in frame could cause their results to fail to replicate or generalize. We also recommend that robots be designed to encourage or discourage certain frames.

==> sections/taxonomy.tex <==
The word "privacy" is used to mean many different things in American English. We take a first crack at it with a taxonomy, which accomplishes two goals: (1) describe the extents or bounds of what we're talking about so we can work towards covering it all in our research program (i.e., towards \emph{content validity}) and (2) gives a more specific definition for each sub-construct so we can refer to them to be more precise. We will use the word "privacy" from now on to refer to all the sub-constructs in our taxonomy. This section lays out our taxonomy of privacy constructs and summarizes the key literature behind it. 

\begin{enumerate}

\item Privacy (see \cite{leino-kilpi_privacy:_2001} for subdivision)
  \begin{enumerate}

  \item Informational (see Prosser (1960) and \cite{solove_understanding_2008} for subdivision)
    \begin{enumerate}
    \item Invasion
    \item Collection
    \item Processing
    \item Dissemination
    \end{enumerate}

  \item Physical
      \begin{enumerate}
      \item Personal Space (\cite{westin_privacy_1967})
      \item Territoriality (\cite{westin_privacy_1967}, \cite{newell_perspectives_1995}, \cite{burgoon_communication_1982}; see \cite{altman_environment_1975} for subdivision)
        \begin{enumerate}
        \item Intrusion
        \item Obtrusion
        \item Contamination
        \end{enumerate}
      \item Modesty (\cite{allen_privacy_2011})
      \end{enumerate}

  \item Psychological
    \begin{enumerate}
    \item Interrogation (\cite{westin_privacy_1967})
    \item Psychological Distance (\cite{hall_hidden_1966})
    \end{enumerate}
    
  \item Social 
    \begin{enumerate}
    \item Association (\cite{allen_privacy_2011})
    \item Crowding/Isolation (\cite{altman_environment_1975})
    \item Public Gaze (\cite{austin_privacy_2003})
    \item Solitude (\cite{allen_privacy_2011}; see \cite{westin_privacy_1967} for subdivision)
    \item Intimacy
    \item Anonymity
    \item Reserve
    \end{enumerate}

  \end{enumerate}
\end{enumerate}

\subsection{The Literature behind the Taxonomy}
We recommend the Stanford Encyclopedia of Philosophy article on privacy by Judith DeCew as a comprehensive guide to the definition of privacy (\cite{decew_privacy_2013}), especially in law and philosophy. Most of the references in this section we owe to the bibliography from that article. 

{\bf 1.a-d} Leino-Kilpi et al. divide privacy as follows \citep{leino-kilpi_privacy:_2001}:

\begin{enumerate}
\item Physical privacy, over personal space or territory
\item Psychological privacy, over thoughts and values
\item Social privacy, over interactions with others and influence from them
\item Informational privacy, over personal information
\end{enumerate}


{\bf 1.a.i-iv} Informational privacy refers to privacy concerns about personal information. Daniel Solove has constructed a taxonomy of privacy concepts based on the work of William Prosser \cite{solove_understanding_2008}. I use the highest level of Solove's hierarchy for 1.a.i-iv. 

{\bf 1.b.i-ii} Privacy could be defined in terms of one's personal space or territory. These concepts are found readily in proxemics literature as well as in psychology and ethology (i.e., animal behavior studies) in general, but are not often connected with privacy. Patricia Newell includes territoriality in her review of \textit{Perspectives on Privacy} (\cite{newell_perspectives_1995}). \cite{leino-kilpi_privacy:_2001} defines physical privacy as being over personal space and territory, and Westin also mentions it when he links human privacy ideas with animal behavior in \cite{westin_privacy_1967}. 

Social psychologist Irwin Altman in \cite{altman_environment_1975} pulls together the related concepts of privacy, personal space, territoriality, and crowding. His book, along with \cite{burgoon_communication_1982}, is a good foundation for \emph{environmental and spatial} factors related to privacy. Judee Burgoon presents a communication perspective on privacy, including territoriality, in a broad survey (\cite{burgoon_communication_1982}). She argues that more ``physical'' privacy could consist of blocking more communication channels, including sight, sound, and even smell (e.g., the smell of food being cooked next door). We would add further channels enabled by technology: phone calls, text messages, Facebook posts, and the like. Alternatively, Burgoon writes that to have more territory, higher-quality territory (e.g., better-insulated walls), and more unquestioned control over that territory is to enjoy more physical privacy. 

{\bf 1.b.iii} Allen lists \emph{modesty} as an important physical privacy concern in medical settings, especially from the philosophical standpoints of Christian ethics and virtue ethics (\cite{allen_privacy_2011}).

{\bf 1.c.i} According to Westin's account of privacy in U.S. law, the right to privacy swelled in the late 1900's (\cite{westin_privacy_1967}). The Supreme Court continued to try cases in which new technologies created privacy concerns beyond physical entry and tangible items. According to Westin, new protections included ``associational privacy'' over group memberships (this is distinct from 1.d.i) and ``political privacy'' over unfair questioning on account of political positions. 

{\bf 1.c.ii} \emph{Proxemics} can include psychological distance as well as physical distance (\cite{hall_hidden_1966} cited by \cite{mumm_human-robot_2011}). Psychological distance is operationalized by things like mutual gaze, smiling, and willingness to answer personal questions.

{\bf 1.d.i and iv} Privacy might also include solitude, i.e., being physically removed from other people. Solitude is more than a freedom from trespassing; one needn't be at home to desire solitude. Anita Allen includes solitude in her article on privacy and medicine (\cite{allen_privacy_2011}). In the medical setting, the sick often want to be comforted by company, but also to have some time alone. This could be especially true for patients with terminal illnesses, who might want to reflect on their lives and make some important decisions. Allen also mentions what she calls ``associational privacy,'' the ability to choose one's own company (\cite{allen_privacy_2011}). She notes that patients do not merely desire intimacy, but rather ``selective intimacy'' with certain loved ones, and this is an aspect of privacy to consider. 

{\bf 1.d.ii} Altman calls both crowding and isolation failures to regulate the amount of interaction with others (\cite{altman_environment_1975}). It may seem odd to call social isolation a privacy issue, but it is a logical conclusion from within Altman's theory of privacy.

{\bf 1.d.iii} To deal with advances in technology, Lisa Austin offers a newer definition of privacy: freedom from ``public gaze'' (\cite{austin_privacy_2003}). Austin is concerned about cases wherein people know they are under surveillance, about the collection of non-intimate but personal information (e.g., in data mining), and about the collection of personal information in public. 

{\bf 1.d.iv-vii} Alan Westin lists four different states of privacy: solitude, anonymity, intimacy (i.e., being alone \emph{with} someone), and reserve (i.e., keeping to oneself) (\cite{westin_privacy_1967}). 
